Most Likely Sequence Generation for $n$-Grams, Transformers, HMMs, and Markov Chains, by Using Rollout Algorithms

In this paper we consider a transformer with an $n$-gram structure, such as the one underlying ChatGPT. The transformer provides next word probabilities, which can be used to generate word sequences. We consider methods for computing word sequences that are highly likely, based on these probabilities. Computing the optimal (i.e., most likely) word sequence starting with a given initial state is an intractable problem, so we propose methods to compute highly likely sequences of $N$ words in time that is a low order polynomial in $N$ and in the vocabulary size of the $n$-gram. These methods are based on the rollout approach from approximate dynamic programming, a form of single policy iteration, which can improve the performance of any given heuristic policy. In our case we use a greedy heuristic that generates as next word one that has the highest probability. We show with analysis, examples, and computational experimentation that our methods are capable of generating highly likely sequences with a modest increase in computation over the greedy heuristic. While our analysis and experiments are focused on Markov chains of the type arising in transformer and ChatGPT-like models, our methods apply to general finite-state Markov chains, and related inference applications of Hidden Markov Models (HMM), where Viterbi decoding is used extensively.

==> recycle.tex <==
In both scales of problems discussed earlier, the sequences selected by the greedy policy have one additional property: starting from any initial state, the sequences quickly reach a cycle of a few states, which repeat itself 






\begin{figure}[t]
\begin{center}
\centerline{{\includegraphics[width=0.6\columnwidth]{1k_greedy_rollout_truncated_rollout.pdf}}}
\caption{Performance of rollout with one-step lookahead and its truncated variant applied to sequence selection problems with $N=1000$ for $50$ randomly generated Markov chains with $1000$ states and $1\%$ branching factor. }
		\label{fig:rollout_small_1k}
		\end{center}
\end{figure}






\begin{figure}[t]
\begin{center}
\centerline{{\includegraphics[width=\columnwidth]{double_rollout_1to5_t.pdf}}}
\caption{Percentage recovery of the optimality loss of the greedy policy through the use of double rollout and its variants, applied to sequence selection problems with $N=100$ for $50$ randomly generated Markov chains with $100$ states and $5\%$ branching factor. Here $\Tilde{\pi}_1$ is rollout with one-step lookahead, $\hat{\pi}_{\ell}$ is double rollout with $\ell$-step lookahead, and $\hat{\pi}_{\ell}^m$ represents $m$-step truncated double rollout for $m=10$ with $\ell$-step lookahead.}
		\label{fig:double_rollout_small}
		\end{center}
\end{figure}
